Heterarchical Granular Dynamics

The two most commonly used methods to model the behaviour of granular flows are discrete element and continuum mechanics simulations. These approaches concentrate on the deterministic description of particle or bulk material motion. Unlike these approaches, this paper introduces an alternative model that describes the stochastic dynamics of the void spaces under the action of gravity. The model includes several key phenomena which are observed in deforming granular media, such as segregation, mixing, and an angle of repose. These mechanisms are modelled heterarchically using both spatial and microstructural internal coordinates. Key aspects of the model include its ability to describe both stable and flowing states of granular media based on a solid fraction cut-off, and the influence of particle size on flow, segregation, and mixing. The model is validated with simulations of column collapse and silo discharge.

==> appendices/shivu.tex <==
\section{Shivu's diffusion --- just for notes, not for publication}

If instead of the above we use Shivu's new measure of diffusivity,

\begin{equation}
    D \propto \frac{\dot\gamma\bar{s}^2}{\sqrt{\phi_\mathrm{cs} - \phi}},
\end{equation}

\noindent this means that $D=\infty$ for solid packings ($\phi=\phi_\mathrm{cs})$, and imaginary for $\phi > \phi_\mathrm{cs}$. %This removes part of the stability criteria for density. We can do the other part by consider the advection velocity more carefully.
I guess this means that the correlation length scale diverges and all of the material gets moved when sheared. This is kind of the opposite of what we need, where we want to have \textbf{no diffusion} when solid. I guess the difference here is that Shivu's model is strain controlled (i.e.\ we always shear at the same \textbf{rate}), whereas ours is more of a mixed condition, where the rate slows down to zero as the material becomes more solid? This is a bit contrary to our idea of things happening \textbf{faster} when the pressure is higher... I'm very confused!

We can add some kind of scaling for $v_y$ with $\phi$. $v_y$ was postulated under the condition that a particle freefalls into a void, and that the size of the void, or what we will now call the mean free path of motion, $l$, is roughly equal to the particle size in a dense medium. We could look for reasonably physical scaling, or begin by noting that such a scaling has the following three conditions:

\begin{enumerate}
    \item At $\phi=1$, $l=0$
    \item At $\phi = \phi_\mathrm{cs}$, $l=\bar s$
    \item At $\phi=0$, $l=\infty$
\end{enumerate}

One simple relationship that satisfies these properties is

\begin{equation}
    \frac{\phi}{\phi_\mathrm{cs}} = \frac{\bar s}{l}
\end{equation}

or

\begin{equation}
    l = \bar s \frac{\phi_\mathrm{cs}}{\phi}
\end{equation}

With this $l$ we then have that

\begin{equation}
    v_y = \sqrt{gl} = \sqrt{g\bar s \frac{\phi_\mathrm{cs}}{\phi}}
\end{equation}

==> appendices/stability.tex <==
\section{Alternative slope stability criterion}\label{app:stability}

which should be equal to the slope of the material at a free surface when the solid fraction of the material is $\nu_\mathrm{cs}$. Note that this second condition is only applied near a free surface (within a distance $L$ of a location with $n=0$, see below for the definition of $L$). The threshold value in (\ref{eq:slope_stability}) can be calculated from a geometric argument by considering that the value of $\nu$ should progress from $\nu_\mathrm{cs}$ to zero in a distance set by $\mu$.

\begin{figure}
    \centering
    \includegraphics{im/slope.pdf}
    \caption{Schematic representation of slope stability criteria.}
    \label{fig:slope}
\end{figure}

As depicted in Figure~\ref{fig:slope}, at the free surface a stable slope is defined by an area where the material is at a density $\nu_\mathrm{cs}$, and proceeds in $K$ drops of density $\Delta\nu$, across a distance $L$, to reach $\nu=0$. Under these conditions

\begin{align}
    K &= \frac{\nu_\mathrm{cs}}{\Delta \nu}, \\
    L &= (K-1)\Delta x.
\end{align}

We can define the slope $\mu$ that corresponds to this configuration by noting that across the distance $L$, the height will drop by $\Delta x$, giving

\begin{equation}
    \mu = \frac{\Delta x}{L}
    % = \frac{\Delta x}{\frac{\nu_\mathrm{cs}}{\Delta \nu}\Delta x - \Delta x}
    = \frac{1}{\frac{\nu_\mathrm{cs}}{\Delta \nu} - 1}.
\end{equation}

Finally, this can be rearranged into an expression for the density difference required to maintain stability at a free surface as

\begin{equation}
    \Delta\nu = \frac{\nu_\mathrm{cs}}{\frac{1}{\mu} + 1}.
\end{equation}

% We note that this method of maintaining a stable slope contains inherent discretisation errors, which are discussed in Appendix~\ref{sec:disc}.
